Error estimates for Euler discretization of high-index saddle dynamics

High-index saddle dynamics provides an effective means to compute the any-index saddle points and construct the solution landscape. In this paper we prove error estimates for Euler discretization of high-index saddle dynamics with respect to the time step size, which remains untreated in the literature. We overcome the main difficulties that lie in the strong nonlinearity of the saddle dynamics and the orthonormalization procedure in the numerical scheme that is uncommon in standard discretization of differential equations. The derived methods are further extended to study the generalized high-index saddle dynamics for non-gradient systems and provide theoretical support for the accuracy of numerical implementations.

==> siam10.tex <==
%% 
%% This is file `siam10.clo', based on size10.clo
%% Revision of siam macros for use with LaTeX 2e
%% 
%% By Paul Duggan for the Society for Industrial and Applied
%% Mathematics. 
%% 
%% October 1, 1995
%%
%% Version 1.0
%% 
%% You are not allowed to change this file. 
%% 
%% You are allowed to distribute this file under the condition that 
%% it is distributed together with all of the files in the siam macro 
%% distribution. These are:
%%
%%  siamltex.cls (main LaTeX macro for SIAM)
%%  siamltex.sty (includes siamltex.cls for compatibility mode)
%%  siam10.clo   (this file)
%%  subeqn.clo   (allows equation numbners with lettered subelements)
%%  siam.bst     (bibliographic style file for use with BibTeX)
%%  docultex.tex (documentation file)
%%  lexample.tex (example file for latex macro) 
%% 
%% If you receive only some of these files from someone, complain! 
%% 
%% You are NOT ALLOWED to distribute this file alone. You are NOT 
%% ALLOWED to take money for the distribution or use of either this 
%% file or a changed version, except for a nominal charge for copying 
%% etc. 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\ProvidesFile{siam10.clo}
              [1994/10/01 v1.0
      SIAM LaTeX file (size option)]
\renewcommand{\normalsize}{%
   \@setfontsize\normalsize\@xpt\@xiipt
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \abovedisplayskip
   \belowdisplayshortskip \belowdisplayskip
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand{\small}{%
   \@setfontsize\small\@ixpt{11}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand{\footnotesize}{%
   \@setfontsize\footnotesize\@viiipt{9.5}%
   \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
   \abovedisplayshortskip \abovedisplayskip
   \belowdisplayshortskip \belowdisplayskip
   \def\@listi{\leftmargin\leftmargini
               \topsep \z@
               \parsep \z@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand{\scriptsize}{\@setfontsize\scriptsize\@viipt\@viiipt}
\newcommand{\tiny}{\@setfontsize\tiny\@vpt\@vipt}
\newcommand{\large}{\@setfontsize\large\@xiipt{14}}
\newcommand{\Large}{\@setfontsize\Large\@xivpt{18}}
\newcommand{\LARGE}{\@setfontsize\LARGE\@xviipt{22}}
\newcommand{\huge}{\@setfontsize\huge\@xxpt{25}}
\newcommand{\Huge}{\@setfontsize\Huge\@xxvpt{30}}
\if@twocolumn
  \setlength\parindent{1em}
\else
  \setlength\parindent{.25in}
\fi
\setlength\headheight{10\p@}
\setlength\headsep   {.2in}
%\setlength\topskip   {10\p@}
\setlength\footskip{.2in}
\if@compatibility 
 \setlength\maxdepth{4\p@}
\else
 \setlength\maxdepth{.5\topskip} 
\fi
\setlength\@maxdepth\maxdepth
\if@compatibility
  \if@twocolumn
    \setlength\textwidth{410\p@}
  \else
    \setlength\textwidth{5.125in}
  \fi
\else
  \if@twocolumn
    \setlength\textwidth{410\p@}
  \else
    \setlength\textwidth{5.125in}
  \fi
\fi
%\if@compatibility\else
%  \@settopoint\textwidth
%\fi
\if@compatibility
  \setlength\textheight{8.25in}
\else
  \setlength\textheight{8.25in}
\fi
%\addtolength\textheight{\topskip}
\if@compatibility
  \if@twoside
     \setlength\oddsidemargin   {.5in}
     \setlength\evensidemargin  {.5in}
     \setlength\marginparwidth {1.25in}
  \else
     \setlength\oddsidemargin   {.5in}
     \setlength\evensidemargin  {.5in}
     \setlength\marginparwidth  {1.25in}
  \fi
  \if@twocolumn
     \setlength\oddsidemargin  {30\p@}
     \setlength\evensidemargin {30\p@}
     \setlength\marginparwidth {48\p@}
  \fi
\else
  \if@twoside
     \setlength\oddsidemargin   {.5in}
     \setlength\evensidemargin  {.5in}
     \setlength\marginparwidth {1.25in}
  \else
     \setlength\oddsidemargin   {.5in}
     \setlength\evensidemargin  {.5in}
     \setlength\marginparwidth {1.25in}
  \fi
  \@settopoint\oddsidemargin
  \@settopoint\marginparwidth
\fi
\if@twocolumn
  \setlength\marginparsep {10\p@}
\else
  \setlength\marginparsep{11\p@}
\fi
\setlength\marginparpush{5\p@}
\if@compatibility
  \setlength\topmargin{\z@}
\else
\setlength\topmargin {\z@}
%  \@settopoint\topmargin
\fi

\setlength\footnotesep{6.65\p@}
\skip\footins 13\p@ \@plus 4\p@ \@minus 2\p@
\setlength\floatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\textfloatsep{20\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\intextsep   {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\dblfloatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\dbltextfloatsep{20\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\@fptop{0\p@ \@plus 1fil}
\setlength\@fpsep{8\p@ \@plus 2fil}
\setlength\@fpbot{0\p@ \@plus 1fil}
\setlength\@dblfptop{0\p@ \@plus 1fil}
\setlength\@dblfpsep{8\p@ \@plus 2fil}
\setlength\@dblfpbot{0\p@ \@plus 1fil}
\setlength\partopsep{\z@}
\def\@listI{\leftmargin\leftmargini
            \parsep \z@
            \topsep \z@
            \itemsep \parsep}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    \z@
              \parsep    \z@
              \itemsep   \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    \z@
              \parsep    \z@
              \partopsep \z@
              \itemsep   \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}
\endinput
%% 
%% End of file `siam10.clo'.
